Physics Constrained Motion Prediction with Uncertainty Quantification

Predicting the motion of dynamic agents is a critical task for guaranteeing the safety of autonomous systems. A particular challenge is that motion prediction algorithms should obey dynamics constraints and quantify prediction uncertainty as a measure of confidence. We present a physics-constrained approach for motion prediction which uses a surrogate dynamical model to ensure that predicted trajectories are dynamically feasible. We propose a two-step integration consisting of intent and trajectory prediction subject to dynamics constraints. We also construct prediction regions that quantify uncertainty and are tailored for autonomous driving by using conformal prediction, a popular statistical tool. Physics Constrained Motion Prediction achieves a 41% better ADE, 56% better FDE, and 19% better IoU over a baseline in experiments using an autonomous racing dataset.

==> 90bicyclemodel.tex <==
\section{Bicycle Model Details}
\label{appendix:bicycle-model}
We define the model as a differential equation $\dot{X} = F(X,u)$. $X = \left[x, y, \theta, v\right]$, and $u = \left[\delta, u\right]$ The only model parameter is $L$, the distance from the center of the front axle to the center of the rear axle. The point $(x,y)$ is at the center of the line segment connecting the centers of the front and rear axles.
\begin{equation}
    \dot{X} = \begin{bmatrix}\dot{x}\\\dot{y}\\\dot{\theta}\\\dot{v}\end{bmatrix} = 
    \begin{bmatrix}
        \left(V+\frac{L}{2}\right)\cos(\theta)\\
        \left(V+\frac{L}{2}\right)\sin(\theta)\\
        \frac{V\tan(\delta)}{L}\\
        a
    \end{bmatrix}
\end{equation}

==> 91errorbounds.tex <==
\section{Integration Error Bounds}
\label{appendix:int-error-bound}
\todo[inline]{Transcribe from my notebook, verify with Wolfram: Update, is this even really relevant?}


To compute the error bounds for Euler integration, we start with our dynamics model:
\begin{equation}
    F(X,u) = \begin{bmatrix}\dot{x}\\\dot{y}\\\dot{\theta}\\\dot{v}\end{bmatrix} = 
    \begin{bmatrix}
        \left(V+\frac{L}{2}\right)\cos(\theta)\\
        \left(V+\frac{L}{2}\right)\sin(\theta)\\
        \frac{V\tan(\delta)}{L}\\
        a
    \end{bmatrix}
\end{equation}
We aim to compute bounds on the expression:
\[\int_0^N F(X,u) dt - NF(X,u)\]


==> 92dynamicfeasbility.tex <==
\section{Dynamic Feasibility}
\label{appendix:dynamic-feasbility}
\todo[inline]{A significantly simpler proof is in the text now}
Here we show that the output trajectory of our method is dynamically feasible, regardless of the input, or the output of the neural network. We define the following components of our network, predicting for N timesteps:
\begin{enumerate}
    \item A neural network $N: I \mapsto \prod_1^N O$
    \item An activation function $A: \prod_1^N O \mapsto \prod_1^N U$ (cartesian product of input space)
    \item A dynamics model $F: X,U \mapsto \dot{X}$
\end{enumerate}
We assume that our initial state $x_0$ is a valid state. Given this initial state and an observation $i$, we represent the output our neural network to be the following recursive expression for t from 1 to $N$
\[
    x_{t} = x_{t-1} + \int_{t}^{t+h} F(x_{t-1},A(N(i))[t])
\]
Note that $A(N(i))$ does not change, but the element of the output that we reference does change.
Trivially, we get that the dynamics model $F$ represents a valid instantaneous change in state. This is because $F$ represents our model dynamics. To get our next step, we calculate the integral of feasible changes in our state from time $t-1$ to $t$, which represents the feasible change in our system from timestep to timestep. Adding this modeled change in our system to the last observed state, must result in another feasible state. We can recursively apply this to show that for all timesteps until $N$, our output is dynamically feasible.

Note that this method assumes that we do not accumulate any integration error. We can further design our activation function $A$ to ensure bounds on our control inputs $U$, for additional control over the ranges of inputs that our dynamics models can get.
